Some Considerations on Universality

The paper puts into discussion the concept of universality, in particular for structures not of the power of Turing computability. The question arises if for such structures a universal structure of the same kind exists or not. For that the construction of universal Turing machines and those with some constraints are presented in some detail.

==> eptcsdata.tex <==
\providecommand{\eid}{11}

